Hybrid-FL for Wireless Networks: Cooperative Learning Mechanism Using Non-IID Data

This paper proposes a cooperative mechanism for mitigating the performance degradation due to non-independent-and-identically-distributed (non-IID) data in collaborative machine learning (ML), namely federated learning (FL), which trains an ML model using the rich data and computational resources of mobile clients without gathering their data to central systems. The data of mobile clients is typically non-IID owing to diversity among mobile clients' interests and usage, and FL with non-IID data could degrade the model performance. Therefore, to mitigate the degradation induced by non-IID data, we assume that a limited number (e.g., less than 1%) of clients allow their data to be uploaded to a server, and we propose a hybrid learning mechanism referred to as Hybrid-FL, wherein the server updates the model using the data gathered from the clients and aggregates the model with the models trained by clients. The Hybrid-FL solves both client- and data-selection problems via heuristic algorithms, which try to select the optimal sets of clients who train models with their own data, clients who upload their data to the server, and data uploaded to the server. The algorithms increase the number of clients participating in FL and make more data gather in the server IID, thereby improving the prediction accuracy of the aggregated model. Evaluations, which consist of network simulations and ML experiments, demonstrate that the proposed scheme achieves a 13.5% higher classification accuracy than those of the previously proposed schemes for the non-IID case.

==> style/__latexindent_temp.tex <==
@article{choi2016millimeter,
  title={Millimeter-wave vehicular communication to support massive automotive sensing},
  author={Choi, Junil and Va, Vutha and Gonzalez-Prelcic, Nuria and Daniels, Robert and Bhat, Chandra R and Heath, Robert W},
  journal={IEEE Commun. Mag.},
  volume={54},
  number={12},
  pages={160--167},
  year={2016},
  Month=dec,
  publisher={IEEE}
}

@inproceedings{DBLP:conf/aistats/McMahanMRHA17,
  author    = {Brendan McMahan and
               Eider Moore and
               Daniel Ramage and
               Seth Hampson and
               Blaise Ag{\"{u}}era y Arcas},
  title     = {Communication-Efficient Learning of Deep Networks from Decentralized
               Data},
  booktitle = {Proc. AISTATS 2017},
  pages     = {1273--1282},
  year      = {2017},
  Month     = apr,
  address   = {Fort Lauderdale, FL, USA},
  timestamp = {Wed, 16 Aug 2017 11:08:55 +0200},
}

@inproceedings{nishio2018client,
  title={Client Selection for Federated Learning with Heterogeneous Resources in Mobile Edge},
  author={Nishio, Takayuki and Yonetani, Ryo},
  booktitle={Proc. IEEE ICC},
  year={2019},
  month=may,
  pages={1--7}
}



@article{zhao2018federated,
  title={Federated Learning with Non-{IID} Data},
  author={Zhao, Yue and Li, Meng and Lai, Liangzhen and Suda, Naveen and Civin, Damon and Chandra, Vikas},
  volume={abs/1806.00582},
  journal={CoRR},
  year={2018},
  month=jun
}



@misc{krizhevsky2009learning,
  title={Learning multiple layers of features from tiny images},
  author={Krizhevsky, Alex and Hinton, Geoffrey},
  year={2009},
  howpublished={Technical report, Univ. of Toronto}
}

@article{Xiao2017FashionMNISTAN,
  title={Fashion-MNIST: a Novel Image Dataset for Benchmarking Machine Learning Algorithms},
  author={Han Xiao and Kashif Rasul and Roland Vollgraf},
  journal={CoRR},
  year={2017},
  month=sep,
  volume={abs/1708.07747}
}

@misc{chollet2015keras,
  title={Keras},
  author={Chollet, Fran\c{c}ois and others},
  year={2015},
  howpublished={\url{https://keras.io}},
}


@misc{ITU-R,
  title={Guidelines for evaluation of radio interface technologies for {IMT-Advanced}},
  author={M. Series},
  year={2009},
  howpublished={Report ITU-R M.2135-1},
}

@ARTICLE{6834753,
author={M. R. Akdeniz and Y. Liu and M. K. Samimi and S. Sun and S. Rangan and T. S. Rappaport and E. Erkip},
journal={IEEE J. Sel. Areas Commun.},
title={Millimeter Wave Channel Modeling and Cellular Capacity Evaluation},
year={2014},
volume={32},
number={6},
pages={1164-1179},
keywords={4G mobile communication;array signal processing;microcellular radio;microwave antenna arrays;millimetre wave antenna arrays;next generation networks;picocellular radio;radio spectrum management;signal detection;space division multiplexing;statistical analysis;submillimetre wave antennas;wireless channels;millimeter wave channel modeling;cellular capacity evaluation;next-generation microcellular wireless network;next-generation picocellular wireless network;radio spectrum management;dimensional antenna array;beamforming;spatial multiplexing;spatial statistical model;dense urban deployment;angular dispersion;spatial cluster;signal detection;4G cellular network;frequency 30 GHz to 300 GHz;frequency 28 GHz;distance 100 m to 200 m;Power measurement;Antenna measurements;Standards;Clustering algorithms;Gain;Delays;Mobile communication;Millimeter wave radio;3GPP LTE;cellular systems;wireless propagation;28 GHz;73 GHz;urban deployments},
doi={10.1109/JSAC.2014.2328154},
ISSN={0733-8716},
month=jun
}

@article{sviridenko2004note,
  title={A note on maximizing a submodular set function subject to a knapsack constraint},
  author={Sviridenko, Maxim},
  journal={Operations Research Letters},
  volume={32},
  number={1},
  pages={41--43},
  year={2004},
  publisher={Elsevier},
  Month=jan
}

@Book{bishop:2006:PRML,
  author = "Christopher M. Bishop",
  title = "Pattern Recognition and Machine Learning",
  publisher = "Secaucus, NJ, USA: Springer-Verlag New York, Inc.",
  year = "2006"
}

@article{hu2015mobile,
  title={Mobile edge computingâ€”A key technology towards 5{G}},
  author={Hu, Yun Chao and Patel, Milan and Sabella, Dario and Sprecher, Nurit and Young, Valerie},
  journal={ETSI white paper},
  volume={11},
  number={11},
  pages={1--16},
  year={2015},
  month=sep
}


@misc{computer-respond-to-this-email,
  howpublished={\url{https://ai.googleblog.com/2015/11/computer-respond-to-this-email.html}},
  author={Greg Corrado},
  title={Computer, respond to this email.}
}


@inproceedings{kannan2016smart,
  title={Smart reply: Automated response suggestion for email},
  author={Kannan, Anjuli and Kurach, Karol and Ravi, Sujith and Kaufmann, Tobias and Tomkins, Andrew and Miklos, Balint and Corrado, Greg and Lukacs, Laszlo and Ganea, Marina and Young, Peter and others},
  booktitle={Proc. ACM SIGKDD 2016},
  pages={955--964},
  year={2016},
  Month=aug,
  address={San Francisco, CA, USA},
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press},
  Month=nov
}

@book{sesia2011lte,
  title={LTE-the UMTS long term evolution: from theory to practice},
  author={Sesia, Stefania and Baker, Matthew and Toufik, Issam},
  year={2011},
  publisher={John Wiley \& Sons}
}

@misc{nasrabadi2007pattern,
  title={Pattern recognition and machine learning: A Matlab Companion},
  author={Bishop, C.M. and Nabney, I.T.},
  Howpublished={Springer, In preparation},
  year={2008},
}

@article{da51a4504fe24a94a3fd90d9b42184cc,
title = "Adaptive subgradient methods for online learning and stochastic optimization",
author = {John Duchi and Hazan, {Elad E.} and Yoram Singer},
year = "2011",
Month = jul,
day = "1",
language = "English (US)",
volume = "12",
pages = "2121--2159",
journal = "Journal of Machine Learning Research",
issn = "1532-4435",
publisher = "Microtome Publishing",
}

@InProceedings{10.1007/978-3-7908-2604-3_16,
author={Bottou, L{\'e}on},
editor="Lechevallier, Yves
and Saporta, Gilbert",
title="Large-Scale Machine Learning with Stochastic Gradient Descent",
booktitle={Proc. COMPSTAT 2010},
year="2010",
Month=aug,
address="Heidelberg, Germany",
pages="177--186",
}

@inproceedings{45648,
title	= {Federated Learning: Strategies for Improving Communication Efficiency},
author	= {Jakub Kone?ný and H. Brendan McMahan and Felix X. Yu and Peter Richtarik and Ananda Theertha Suresh and Dave Bacon},
year	= {2016},
Month = dec,
booktitle	= {Proc. NIPS Workshop on Private Multi-Party Machine Learning}
}


@inproceedings{Bonawitz2017,
 author = {Bonawitz, Keith and Ivanov, Vladimir and Kreuter, Ben and Marcedone, Antonio and McMahan, H. Brendan and Patel, Sarvar and Ramage, Daniel and Segal, Aaron and Seth, Karn},
 title = {Practical Secure Aggregation for Privacy-Preserving Machine Learning},
 booktitle = {Proc. ACM CCS},
 year = {2017},
 month={Oct.},
 isbn = {978-1-4503-4946-8},
 location = {Dallas, Texas, USA},
 pages = {1175--1191},
 numpages = {17},
 doi = {10.1145/3133956.3133982},
 acmid = {3133982},
 keywords = {federated learning, machine learning, privacy-preserving protocols, secure aggregation},
}

@article{Geyer2017,
  author    = {Robin C. Geyer and
  				Tassilo Klein and
                Moin Nabi},
  title     = {Differentially Private Federated Learning: A Client Level Perspective},
  journal   = {CoRR},
  volume    = {abs/1712.07557},
  year      = {2017},
}

@inproceedings{Konecny2016,
  author    = {Jakub Konecn{\'{y}} and
               H. Brendan McMahan and
               Felix X. Yu and
               Peter Richt{\'{a}}rik and
               Ananda Theertha Suresh and
               Dave Bacon},
  title     = {Federated Learning: Strategies for Improving Communication Efficiency},
booktitle={Proc. NIPS Workshop on Private Multi-Party Machine Learning},
month={Dec.},
year={2016}
}

@article{wang2019adaptive,
  title={Adaptive federated learning in resource constrained edge computing systems},
  author={Wang, Shiqiang and Tuor, Tiffany and Salonidis, Theodoros and Leung, Kin K and Makaya, Christian and He, Ting and Chan, Kevin},
  journal={IEEE J. Sel. Areas Commun.},
  volume={37},
  number={6},
  pages={1205--1221},
  year={2019},
  month=jun,
  publisher={IEEE}
}

@inproceedings{Nishio13,
 author = {Nishio, Takayuki and Shinkuma, Ryoichi and Takahashi, Tatsuro and Mandayam, Narayan B.},
 title = {Service-oriented Heterogeneous Resource Sharing for Optimizing Service Latency in Mobile Cloud},
 booktitle = {Proc. First International Workshop on Mobile Cloud Computing \& Networking},
 year = {2013},
 month=july,
 pages = {19--26},
 location = {Bangalore, India},
 address = {Bangalore, India},
}

@ARTICLE{Zeng16,
author={D. {Zeng} and L. {Gu} and S. {Guo} and Z. {Cheng} and S. {Yu}},
journal={IEEE Trans. Computers},
title={Joint Optimization of Task Scheduling and Image Placement in Fog Computing Supported Software-Defined Embedded System},
year={2016},
volume={65},
number={12},
pages={3702-3712},
month=dec
}

@article{sattler2019robust,
  title={Robust and communication-efficient federated learning from non-iid data},
  author={Sattler, Felix and Wiedemann, Simon and M{\"u}ller, Klaus-Robert and Samek, Wojciech},
  volume={abs/1903.02891},
  journal={CoRR},
  year={2019},
  month=mar
}

@article{yang2019scheduling,
  title={Scheduling policies for federated learning in wireless networks},
  author={Yang, Howard H and Liu, Zuozhu and Quek, Tony QS and Poor, H Vincent},
  volume={abs/1908.06287},
  journal={CoRR},
  year={2019},
  month=oct
}
